JiuZhang 2.0: A Unified Chinese Pre-trained Language Model for Multi-task Mathematical Problem Solving

Although pre-trained language models~(PLMs) have recently advanced the research progress in mathematical reasoning, they are not specially designed as a capable multi-task solver, suffering from high cost for multi-task deployment (\eg a model copy for a task) and inferior performance on complex mathematical problems in practical applications. To address these issues, in this paper, we propose \textbf{JiuZhang~2.0}, a unified Chinese PLM specially for multi-task mathematical problem solving. Our idea is to maintain a moderate-sized model and employ the \emph{cross-task knowledge sharing} to improve the model capacity in a multi-task setting. Specially, we construct a Mixture-of-Experts~(MoE) architecture for modeling mathematical text, so as to capture the common mathematical knowledge across tasks. For optimizing the MoE architecture, we design \emph{multi-task continual pre-training} and \emph{multi-task fine-tuning} strategies for multi-task adaptation. These training strategies can effectively decompose the knowledge from the task data and establish the cross-task sharing via expert networks. In order to further improve the general capacity of solving different complex tasks, we leverage large language models~(LLMs) as complementary models to iteratively refine the generated solution by our PLM, via in-context learning. Extensive experiments have demonstrated the effectiveness of our model.

==> model_backup.tex <==
\section{Preliminary}

\subsection{Problem Statement}
We first formally describe  \emph{mathematical text},  a general phrase referring  to the text relating to a mathematical problem. 
In our corpus,  a mathematical problem is associated with two texts, namely problem statement and solution text (\aka answer key). 
The problem statement introduces necessary background information and explains the problem that is to be solved, and  the answer key describes the key hints or complete solving  procedure for deriving the answer. 
We concatenate both  problem statement and solution description as the \emph{mathematical text} of a mathematical problem. 

Overall, a mathematical text is a  textual description that mixes text words with math symbols. Given a mathematical problem $q$, the corresponding mathematical text can be considered as a sequence of $n$ tokens, denoted as $q=\{t_1, t_2, \cdots , t_n\}$, where each token $t_i$ is either a text word or a math symbol (denoting a variable or an operator).  Furthermore, a consecutive segment of $l$ math symbols constitute a math formula, denoted as $f_i = \{s_1, \cdots, s_l\}$, where each math symbol $s_j$ is from $\{t_1, t_2, \cdots , t_n\}$. There are usually multiple formulas in a mathematical text, denoted as $\{f_1, f_2, \cdots , f_m\}$.

Based on the above notations, this work focuses on pre-training a PLM on a large-scale corpus consisting of  
mathematical texts. Then, the PLM can be 
fine-tuned on various mathematical tasks (\eg knowledge point classification and similar question retrieval), and improve the corresponding task performance.




\section{Approach}
In this section, we first introduce the backbone of our approach Jiuzhang, and then present the mixture-of-experts multi-task training and in-context learning via large language models.


\begin{figure*}
  \centering
  \includegraphics[scale=0.6]{figure/model.pdf}
  \caption{The overview of our approach.}
  \label{approach}
\end{figure*}

\subsection{Backbone: JiuZhang}
% zbc
JiuZhang is a Chinese pre-training model for mathematical problem understanding. The model architecture of JiuZhang consists of a shared encoder and two task-specific decoders to deal with understanding and generation tasks. Based on the model architecture, JiuZhang is pre-trained with a curriculum pre-training strategy, which helps JiuZhang gradually learn mathematical knowledge and logic from easy to difficult.

\subsubsection{Architecture}
The basic architecture of JiuZhang consists of a shared encoder, a decoder for understanding tasks ($U$-decoder), and a decoder for generation tasks ($G$-decoder).
The shared encoder and the $U$-decoder are bidirectional Transformers, and the representation of the ``\textsf{[CLS]}'' token at the last layer of the $U$-decoder will be used for representing the input sequence in understanding tasks.
The $G$-decoder is an auto-aggressive Transformer, and is trained by the teacher-forcing algorithm for generation tasks.
Note that the two task-specific decoders have fewer layers compared to the shared encoder (\ie 2 layers \emph{v.s.} 10 layers).
In this way, the shared deep encoder plays the key role of producing general representations of the input data, and the two shallow decoders mainly focus on accomplishing specific tasks.
%Thus, the number of involved parameters for a single task is comparable to the original scale of PLM architecture~\cite{devlin-etal-2019-bert}. Moreover, the decoding efficiency of generation tasks is improved benefiting from fewer decoder layers.

Given a mathematical problem $q=\{t_1, \cdots, t_{n}\}$, a shared encoder is adopted to encode mathematical semantic information into contextualized token representation $\{\mathbf{h}^{(L)}_{1}, \mathbf{h}^{(L)}_{2}, \cdots, \mathbf{h}^{(L)}_{n}\}$. %The shared encoder provides general mathematical semantics for different math-related tasks.
Then, the $U$-decoder and $G$-decoder will solve the understanding tasks and the generation tasks based on the token representations, respectively. 

%The $U$-decoder is a shallow bidirectional Transformer for understanding tasks. Following BERT~\cite{devlin-etal-2019-bert}, a special symbol ``\textsf{[CLS]}'' is inserted at the beginning of the input sequence. 

\subsubsection{Pre-training Tasks}
A curriculum pre-training strategy is proposed for helping JiuZhang learn mathematical knowledge and logic from basic to advanced courses. 
The pre-training is divided into three stages, and the three stages mainly adopt the masked token prediction tasks, mathematical logic recovering tasks, and solution checking tasks, respectively.
%First, the basic course utilizes masked language models and denoised auto-encoding tasks to learn fundamental mathematical semantics. Next, JiuZhang adopts an advanced course that focuses on reconstructing shuffled sentences and formulas to further enhance the understanding of mathematical logic. Lastly, a challenging solution-checking task is proposed to increase the model's ability to detect and correct errors in its own generated outputs.

\paratitle{Basic Course: Masked Token Prediction.}
The basic course aims to enhance the basic understanding of math symbols and establish semantic connections between math symbols and textual words. Given a mathematical text, 15\% tokens of the input sequence are selected for masking (including both words and symbols), in which 80\% ones are replaced by the token ``\textsf{[MASK]}'', 10\% ones are replaced by a random token and the rest 10\% ones remain unchanged. Let $\widetilde{x}$ denote the masked sequence,  $V_{mask}$ denote the selected tokens, and the MLM and DAE losses are defined as:
\begin{align}
     L_{MLM} &=\sum_{t_i \in V_{mask}}-\log{p(t_i | \widetilde{x};\Theta_{E}, \Theta_{U})},
    \label{eq-mlm}\\
     L_{DAE} &=\sum_{i}-\log{p(t_i|t_{<i}, \widetilde{x};\Theta_{E}, \Theta_{G})},
    \label{eq-dae}
\end{align}
where $p(t_i | \widetilde{x};\Theta_{E}, \Theta_{U})$ and $p(t_i|t_{<i};\widetilde{x};\Theta_{E}, \Theta_{G})$ denote the prediction probabilities of the token $t_i$ at the $i$-th position according to $U$-decoder and $G$-decoder, respectively.
Besides, based on the causality of math solution, we also devise a linearly increasing weighting mechanism that assigns larger masked probability in larger positions.
\ignore{
Based on the causality of math solution, a linearly increasing weighting mechanism that assigns larger masked probability in larger positions is utilized in masking tokens:
\begin{equation}
    s_i = \frac{30}{n-1} \times i,
    \label{eq-mask}
\end{equation}
where $ s_i$ is the sampling weight to be masked for the $i$-th position, $n$ is the sentence length, and $i$ is the position index ranging from 0 to $n-1$.} 

\paratitle{Advanced Course: Mathematical Logic Recovering.}
% The basic course enables JiuZhang to gain a fundamental understanding of mathematical symbols and descriptive language at the token level. 
To fully comprehend mathematical problems and the logical derivations necessary, logic-based pre-training tasks are proposed with the reconstruction of shuffled sentences and formal statements. 
For the Shuffled Sentences Recovering (SSR) task, the sentences in the solution text (denoted as $d$) are shuffled, producing a corrupted solution text denoted as $\widetilde{d}_{S}$. The pre-training objective is to recover the original solution text $d$ based on $\widetilde{d}_{S}$ with $G$-decoder:
\begin{equation}
    L_{SSR}=\sum_{i}-\log{p(t_i|t_{<i},  \widetilde{d}_{S};\Theta_{E}, \Theta_{G}} ),
    \label{eq-ssr}
\end{equation}

For the Shuffled Formulas Recovering~(SFR) task, he formulas $\{f_1, f_2, \cdots , f_m\}$ from the solution text are shuffled to construct the corrupted solution text denoted as $\widetilde{d}_{F}$. The PLM aims to recover the original text based on $\widetilde{d}_{F}$:
\begin{equation}
    L_{SFR}=\sum_{i}-\log{p(t_i|t_{<i}, \widetilde{d}_{F};\Theta_{E}, \Theta_{G}}).
    \label{eq-sfr}
\end{equation}

\paratitle{Advanced Course: Solution Checking}
To improve the sensitivity of PLMs to solution errors, the Dual-Decoder Solution Checking~(SC) task is adopted as an advanced course. First, the two decoders are utilized to fill the masked symbols or words. Then, they are trained to detect and correct the solution generated by each other.

Specifically, given the solution text $d=\{t_1,t_2,\cdots,t_l\}$, a proportion of tokens following the same strategy in the basic course  are selected to produce the masked text $\widetilde{x}$.
Then, the $U$-decoder and $G$-decoder generate recovered results based on their own generation probabilities of the masked tokens $\widetilde{d}_{U}$ and $\widetilde{d}_G$.
Next, the generated texts $\widetilde{d}_{G}$ and $\widetilde{d}_U$ are then evaluated and corrected by the $U$-decoder and $G$-decoder. Therefore, errors in generations will be detected and corrected through a dual process. Such a pre-training process can be formulated as:
\begin{align}
    L_{USC} &= \sum_{i}-\log{p(t_i|\widetilde{d}_G;\Theta_{E},\Theta_{U})}, \label{eq-usc}\\%;\hat{d}_U)}, \\
    L_{GSC} &=\sum_{i}-\log{p(t_i|t_{<i},
    \widetilde{d}_U;\Theta_{E},\Theta_{G})}, %;\hat{d}_G)},
    \label{eq-gsc}
\end{align}
where $L_{USC}$ and $L_{GSC}$ denote the self-correction losses for the $U$-decoder and $G$-decoder, respectively.

%The correction pre-training task enables PLMs to verify the accuracy of all crucial steps in the solution process, particularly in the context of complex mathematical problems that entail long solving steps.

\subsection{Multi-task Training with Mixture-of-Experts}
To decompose and capture the shared mathematical knowledge across different tasks, we borrow the idea of Mixture-of-Experts~(MoE)~\cite{} into Jiuzhang and propose the multi-task training approach.
In this part, we first describe how to add the MoE module into Jiuzhang, and then present the multi-task continual pre-training and fine-tuning based on the MoE-enhanced model architecture.
%the structure of MoE. Then we go into detail on how to use MoE in continue pre-training and multi-task fine-tuning. 

\subsubsection{Adding MoE into Jiuzhang}
MoE~\cite{} is a widely used technique that adopts multiple expert networks to divide the latent space into several regions.
Generally, all the expert networks share the same structure but have different parameters, with a routing (or gating) mechanism that assigns individual inputs into a few proper experts among all the candidates.
To integrate MoE into Jiuzhang, we aim to reuse the pre-trained parameters of Jiuzhang and add MoE layers.
Concretely, we replace the feed-forward layer in the shared deep encoder of Jiuzhang by the MoE layer, since the shared deep encoder mainly focuses on generating general representations.

%We first describe the basic structure of MoE and then provided the detail information on how to use MoE better.

\paratitle{MoE Layer.}
As the shared deep encoder is composed by multiple bidirectional Transformer layers, we add the MoE layer in each Transformer layer to substitute for the feed-forward layer.
Each MoE layer consists of a routing network $R(\cdot)$ and multiple expert networks $\{E_{i}(\cdot)\}_{i=1}^{K}$, where $K$ denotes the number of expert candidates.
To prevent drastically changes on the latent space of Jiuzhang, we utilize the parameters of the original feed-forward layer to initialize the parameters of the multiple expert networks.
Following existing works~\cite{}, we adopt the token-wise routing mechanism that assigns experts individually for each token.
%JiuZhang encoder layer consists of self-attention and feed forward network. We treat feed forward network as expert and define Mixture-of-Experts (MoE) layer as a group of experts $\{E_i\}_{i=1}^n$. 
%Any feed forward network in JiuZhang encoder is replaced with MoE. 
%Each expert has the same structure, but has different parameters and focus on different abilities. 
Given an input mathematical problem $q=\{t_1, \cdots, t_n\}$, in each Transformer layer, the multi-head self-attention layer will first produce the aggregated representations of all these tokens $\{\bm{h}_1, \cdots, \bm{h}_n\}$.
Then, for each token, the routing network will generated the estimated probability distribution on the $K$ experts as:
%we utilize a gating network $G$ to select the appropriate experts. MoE first uses the gating network to obtain an output vector $G(h) \in \mathbb{R}^n$, which is the probability distribution on $n$ experts, indicating the score of different experts on the token $h$:
\begin{align}
    R(\bm{h}) = \text{softmax}(\bm{W}_r \cdot e(\bm{h})), 
    \label{eq-gating-network}
\end{align}
where $\bm{W}_r$ is the trainable matrix and $e(\cdot)$ is the encoding function to map the token representation into the input of the routing network, which can be revised for injecting other conditions (\eg training task). 
Next, we incorporate the sparse activation mechanism~\cite{} to select and utilize few expert networks. 
Specifically, according to the estimated probability distribution vector $R(\bm{h})$, we rank all the experts networks only select the top-$k$ (usually $k=1$) ones to encode the token representation and make weighted summation on their outputs to obtain the output of the MoE layer:
\begin{align}
    MoE(\bm{h}) = \sum_{i=1}^{k}{R(\bm{h})_i \times E_{i}(\bm{h})}. 
    \label{eq-gating-network}
\end{align}

\subsubsection{Continual Multi-task Pre-training with MOE}
% JiuZhang使用基于课程学习的预训练，依次进行基础课程和高级课程的学习，在预训练结束时，取得了较好效果。但是不同的预训练任务对应不同的数学能力，但是分阶段的预训练将不同的能力割裂开来，并且在几个不同的任务中使用相同的共享权重，不利于模型的训练。因此我们将三个预训练任务混合在一起，完成一个多任务连续预训练，使MoE从预训练任务中吸收知识。
Although the MoE layers reuse the parameters of the feed-forward layers, they also need to be pre-trained to better adapt into the whole architecture of Jiuzhang.
Therefore, we devise the continual multi-task pre-training process that reuses the pre-training tasks of Jiuzhang, to warm up the MoE layers for decomposing and capturing shared mathematical knowledge points across these tasks.

\paratitle{Multi-task Objective.}
As mentioned in Section~\ref{}, Jiuzhang utilizes the curriculum pre-training strategy that progressively learns three types of pre-training tasks, corresponding to different mathematical abilities from basic to advanced.
In fact, since these pre-training tasks are based on the same pre-training corpus, for the same instance, they may also share the same mathematical knowledge points to predict the masked tokens, recover shuffled formulas and correct the generated solutions.
Therefore, we directly integrate them in a multi-tasking manner, and the training objective is
\begin{align}
    L_{MT} = L_{MLM} + L_{DAE} + L_{SSR} + L_{SFR} + L_{USC} + L_{GSC},
    \label{eq-continue-pretrain}
\end{align}
where the input and output data formats are the same as in Section~\ref{}.
For implementation, given a batch of instances, we first randomly select a half of ones for the masked token prediction task and the other ones for the mathematical logic recovering task, due to their different data formats.
Then, the solution checking task will be performed to correct the predicted tokens or recovered text for the two halves of instances, respectively.
In this way, we can train the expert networks in MoE layers to characterize the shared mathematical knowledge across the three types of pre-training tasks.

\paratitle{Sparsely Routing with Jitter Noise.}
%There are two options for routing functions: token-level function and task-level function. 
To save the computational cost in MoE layers, given the token representation of each token $\bm{h}$, we encode it only by the expert network with the top-$1$ estimated probability using Eq.~\ref{eq-gating-network}, where we set $e(\bm{h})=\bm{h}$ for convenience. 
In this way, for each instance, the computational cost of the expert network is the same as the original feed-forward layer in original Jiuzhang.
However, existing works~\cite{fedus2021switch} have revealed that such a sparse expert assignment approach would deterministically choose the top-$1$ expert, causing the expert network easy to overfit.
Therefore, we introduce randomness into the expert selection process by using the jitter noise~\cite{fedus2021switch} in the routing network.
The jitter noise $\epsilon_j$ is a randomly scaling distribution vector that will be multiplied by the estimated probability distribution as:
\begin{align}
    R(\bm{h}) = \text{softmax}(\bm{W}_r \cdot \bm{h} \cdot \epsilon_j), 
    \label{eq-jitter-noise}
\end{align}
%following William ~\etal~\cite{}, to explore the expert assignment approach more fully rather than deterministically selecting the top expert, we use multiplication jitter noise in gating network:
where $\epsilon_j$ is randomly sampled from a uniformly distribution as $[1-\eta, 1+\eta]$ and $\eta$ is the hyper-parameter to control the noise scale.
In this way, the probability scores of different experts would be increased or decreased randomly, enforcing the expert networks being more robust to perturbations on the routing results.


\paratitle{Auxiliary Losses.} 
There are two problems that would be frequently encountered for MoE methods and affect the performance, \ie the unbalanced load among experts~\cite{} and the training instability~\cite{}.
To alleviate these problems, we follow existing works~\cite{} and adopt two auxiliary losses as the regularizer terms in our approach.
The unbalanced load problem refers that a certain expert is extremely frequently routed, which may cause the overfitting problem on this expert and the underfitting problem on other experts.
Therefore, we focus on improving the uniform routing among all $K$ experts.
Concretely, we encourage the accumulated estimated probabilities for each expert to be uniform, denoted as:
\begin{align}
    L_{UL} = \alpha \cdot K \cdot \sum_{i=1}^{K}{f_i \cdot P_i},
    \label{eq-auxiliary-1}
\end{align}
where $f_i$ is the number of tokens dispatched to the expert $i$, and $P_i$ is the accumulated routing score estimated by the routing network for the expert $i$, $\alpha$ is the coefficient to control the influence.
This loss encourages uniform routing since it is minimized under a uniform distribution. 
The training instability problem is generally caused by the great volatility of the routing scores froom the routing network.
Thus, we leverage the Z-loss~\cite{} that encourages the routing logits of all tokens to remain small as:
\begin{align}
    L_Z = \frac{1}{T} \log \sum_{i=1}^{n} \exp(R(\bm{h}_i))^2
    \label{eq-auxiliary-3}
\end{align}

 




%\paratitle{JiuZhang-MOE.} 
% top-1， softmax，expert-capacity，router, fix temp，参数量对比，计算量对比
% 一个JiuZhang-MoE从课程学习预训练好的JiuZhang上建立。为了在不同任务之间更好的共享数学知识，我们进一步使用MoE改进JiuZhang模型，将共享编码器中的前馈网络(FFN)替换为MoE FFN。我们使用令牌级路由器机制，由每个token的representation作为路由网络的输入，来确定该token与expert的分数。具体为$R(h)=x_i$，这种令牌级路由器可以根据令牌本身灵活选择专家(如数字令牌，更可能需要计算能力)。然后使用稀疏激活的expert，即选择top-1分数的expert进行激活。同时我们还保持温度不变
% \textcolor{red}{This section seems more appropriate for implementation details. }
%In order to better share mathematical knowledge between different tasks, Jiuzhang-Moe is built on curriculum pre-trained JiuZhang. We replace the feed forward network (FFN) in the shared encoder with MoE. 


%\paratitle{Multi-task Learning} 
% 我们将基础课程和高级课程以多任务形式结合起来，继续预训练JiuZhang-MoE。一个batch里每个样本随机进行Masked Token Prediction或Mathematical Logic Recovering任务，所有样本都会进行 Solution Checking。loss如下：xxxx.通过多任务继续预训练，不同任务之间共享的数学知识被打通。



\subsubsection{Multi-task Fine-tuning via MoE}
After multi-task continual pre-training, Jiuzhang with the MoE layers has decomposed and absorbed different mathematical knowledge points from the pre-training tasks. 
For applying to downstream math-related downstream tasks, we also propose the multi-task fine-tuning strategy to share and utilize the useful knowledge across the available annotations from these tasks, for further improving the performance.

%Thus we utilize a prompt-based multi-task fine-tuning method, using MoE to further absorbe downstream task knowledge. 
\paratitle{Unifying Fine-tuning Tasks.}
For multi-task fine-tuning, we combine the available math-related downstream tasks together to jointly fine-tune the parameters of our model.
Such a way can characterize the useful knowledge across different tasks, and also endow our model the capacity of jointly solving multiple tasks.
However, the formats of the input and output data for downstream tasks are generally different, making it hard to be directly combined.
Fortunately, our backbone Jiuzhang has two decoders that can handle both natural language understanding and generation tasks.
Therefore, we can unify the above math-related tasks into either the general NLU or NLG format.
Concretely, for all text classification tasks, we can collect their annotated labels together and convert them into a super multi-label classification task.
In this way, we can integrate our U-decoder with a super multi-label classifier head to accomplish all these classification tasks.
For all text generation tasks, we can directly reuse their original input and output texts and leverage the G-decoder to solve them.
To better distinguish the different tasks for our model, given the training data from $m$ tasks, we also devise $m$ task prompt embeddings, denoted as $\{\bm{t}_1, \cdots, \bm{t}_m\}$.
For each instance, we insert its task prompt embedding after the $\textsc{[Cls]}$ token embedding.


\paratitle{Routing with Task Prompt.}
During multi-task fine-tuning, as the task type may also determine the utilization of different mathematical knowledge points belong to different experts, we aim to revise the routing mechanism to introduce the task-level conditions.
Specially, in each MoE layer, we add the input token representation $\bm{h}$ with the representation of the task prompt $\bm{t}$, to compose the input of the routing layer for estimating the probability distribution on all experts as:
\begin{equation}
    R(\bm{h}) = \text{softmax}(\bm{W}_r \cdot (\bm{h}+\bm{t}) \cdot \epsilon_j), 
    \label{eq-ft-routing}
\end{equation}
where we also utilize the jitter noise strategy to improve the robustness.
%mechanism can explicitly consider task information in routing mechanism.

%\paratitle{Multi-task Learning.}
% 在下游任务里有生成和分类两种任务，我们以多任务学习的方式在这些任务上进行统一的微调。具体使用异构batch方法，即一个batch里有来自多个任务的样本
%In downstream tasks, there are two types of tasks: generation and classification. We use formulate these tasks as multi-task learning to fine-tune them. We use a heterogeneous batch method~\cite{}, where exists samples from different tasks in a batch. 

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\linewidth]{figure/prompt.pdf}
%	\caption{The English version of our prompt template used to in-context learning. Chinese prompt and instruction will be used in practice.}
%	\label{LLM-framework}
%\end{figure}

\subsection{Iteratively Refining Results via Large Language Models}
%Based on the multi-task training with MoE layers to characterize the shared mathematical knowledge points across various math-related tasks, we further consider to improve the quality of the generated texts by our approach via large language models~(LLMs).
Actually, due to the limitation of pre-training data, existing PLMs are easy to make mistakes during generation, \eg calculation error and transcription error.
Such a problem can be solved by large language models, since they have been pre-trained on large-scale general corpus, owning better capacity of generating fluent and logically correct texts.
To effectively leverage the LLM, we propose to utilize the in-context learning method~\cite{} to guide the LLM to iteratively refine the generated results of our model.
To achieve it, the key is to compose high-quality prompts as the input to instruct the LLM, which generally consist of a clear instruction and few sampled helpful examples as reference.
In our approach, we first design a retrieval strategy to select the most relevant exemplars for constructing the prompts, and then devise an iterative prompting method that switches instructions to progressively correct the generated results.

%a set of retrieval methods and prompt templates to retrieve relevant exercises and construct prompts.
%Then, we select different retrieval methods and prompt templates each time to build prompts to call the large language model to iteratively revise the imperfect generations.

\subsubsection{Constructing Prompts using Retrieved Samples}
%In a certain iteration round, our approach aims to correct the specific errors of the previous iteration's generation by prompting LLM with specific prompts.
Since existing LLMs are not specially designed for Chinese mathematical problem understanding, it has not sufficiently learned the necessary knowledge points to effectively accomplish Chinese math-related tasks.
Therefore, we mainly leverage them as the complementary model to refine the generated results by our model, to fully utilize their strong generation capacity.
Formally, given the mathematical problem $q$, we first utilize Jiuzhang with MoE layers to generate the analysis $a'$ to answer it, and the LLM will be utilized to refine $a'$ into $\tilde{a}$ to improve its quality.
To provide effective guidance on the LLM, we construct the prompts with few retrieved relevant exemplars and hand-craft natural language instructions.

\paratitle{Retrieving Exemplars.}
As empirical studies~\cite{} have revealed that the exemplars in the prompts of LLMs are important to the task performance, we adopt an unsupervised text retrieval model, SimCSE~\cite{} to select the most relevant instances from the training data as the exemplars.
SimCSE incorporates the Dropout mechanism to augment positive representations and utilizes the contrastive learning objective for training.
For implementation, we utilize our Jiuzhang initialization, and fine-tune it via SimCSE method.
In the retrieval stage, given the mathematical problem $q$ and the training data set as the retrieval candidate pool $D = \{(q_i, a_i)\}^n_{i = 1}$, we first encode them into dense vectors by SimCSE, and then sample the top-$n$ relevant exemplars $C = \{(q_j, a_j)\}^n_{j = 1}$ based on the cosine similarity score, \ie $s(q, q_i) = cos(E(q), E(q_i)$, where $E(\cdot)$ denotes the output embedding of the $\textsc{Cls}$ token by SimCSE.

%since we found that when solving complex mathematical problems, the performance of LLM is extremely dependent on the similarity between the exemplars and the current problem. And we manually designed special prompt templates to guide the LLM to revise the generated results rather than solve the problem itself.



\paratitle{Building Prompts.}
In order to guide the LLM to refer to the retrieved exemplars for revising the generated result $a'$ from Jiuzhang, our devised input of the LLM consists of four parts, \ie the given question $q$, the generated result $a'$, retrieved exemplars $C=\{(q_j, a_j)\}^n_{j=1}$ and a natural language instruction $I$.
Simply, we concatenate the above texts into a long sentence, to compose the prompt template as:
\begin{equation}
    [q; a'; C; I]
    \label{build_prompt}
\end{equation}
Based on this template, we can freely change the instruction $I$ and iteratively update the refined result $a'$, to progressively improve the quality.


\subsubsection{Iterative Prompting for Results Refining}
% czp
Generally, the generated results from PLMs may suffer from many kinds of mistakes, \eg inconsistent logic and language typos, hence it is hard for the LLM to completely check and correct all these mistakes at once.
Therefore, we devise a three-stage iterative refining strategy that gradually improves the quality of the generated results following the coarse-to-fine manner.
Concretely, we design three instructions for the three stages to guide the LLM that focuses more on refining the overall logic, incorrect deductions and improper language expressions, respectively.
We show the above instructions in Table~\ref{tab:commands}.
Besides, to better cooperate with the above instructions, we also revise the way of retrieving exemplars.
In the first stage, we only rely on the problem statement $q$ for finding similar questions and refer to their overall logic.
In the second stage, we leverage both $q$ and the generated analysis $a'$ for retrieving helpful questions with similar analysis to check the deduction process.
In the third stage, we only utilize the generated analysis $a'$ for retrieval, to find other similar analysis for correcting possible improper language expressions.

In our experiments, we have found that only one-turn iteration in each stage is not enough to accomplish the corresponding stage objective.
Therefore, we perform $T$-step iterations for each stage.
In the $t$-th step, the output refined analysis $\Tilde{a}^{(t)}$ will be used as $a'^{(t+1)}$ in the next step to compose the input and the retrieved exemplars can also be updated according to $a'^{(t+1)}$.
In this way, we can iteratively refine the generated results until solving the targeted issue in each stage, and finally generate more high-quality results.

\ignore{
The process of iteratively answer correction can be divided into three stages: Idea Correction Stage, Error Correction Stage and Language Expression Correction Stage. 
Each stage has unique retrieval methods and prompt templates and will repeat several times.
Formally, we design a set of retrieval methods and prompt templates, denoted as $R=\{r_1, r_2, r_3\}$ and $P=\{p_1, p_2, p_3\}$ respectively. 
The $t$-th stage uses $r_t$ as a retrieval method and uses template $p_t$ to construct a demonstration to prompt LLM. 
Each stage has a hyper-parameter $k$, which means the iteration steps of the corresponding stage.
The three stages of answer correction instruct LLM to revise JiuZhang's solution step by step ranging from coarse to fine-grained. The details of retrieval methods and instructions in each stage prompt are shown in Table~\ref{iter-setting}.

\paratitle{Idea Correction Stage}
For each mathematical problem $q$, the problem content $c$ is used to retrieve similar problem in this stage. 
The problem content $c$ will be encoded by the word2vector model to a vector $v_c \in \mathbb{R}^d$ as the embedding of the problem to retrieve similar problems from the retrieval set.
It's empirical that little difference in the content will lead to differences in the ideas for solving problems most of the time.
Using problem content as key of retrieval can retrieve similar problem description and diversified solution from retrieval set.
The corresponding instruction in the prompt guides LLM to select correct idea for the problem.

\paratitle{Error Correction Stage}
In this stage, we use problem content $c$ and analysis (proper analysis for retrieval set problems while generated analysis for test set problems) to retrieve examplars.
The vector $v_c \in \mathbb{R}^d$ and $v_a \in \mathbb{R}^d$ are represented the embedding of problem content and analysis respectively.
The final embedding of a problem $v \in \mathbb{R}^{2d}$ used in retrieval is the concatenating of content embedding $v_c$ and analysis embedding $v_a$.
The concatenating of $v_c$ and $v_a$ forces the retriever to retrieve problems which have similar problem content and analysis with the test problem.
During this stage, we provide more related problems both in problem description and idea of solution as examplars to LLM.
This stage helps LLM to correct the calculation errors and logic errors in the generated analysis from the last iteration.

\paratitle{Language Expression Correction Stage}
Given a mathematical problem of test set, its analysis is generated by JiuZhang and corrected by LLM through the first two stages.
So the target of the third stage is to improve the fluency of generated analysis and correct the remaining errors in it.
We encode problem analysis (generated analysis for problem in test set) to an embedding $v_a \in \mathbb{R}^d$ and use it to retrieve the examplars.
The examplars provided to LLM in this stage have high similarity in analysis with problems in test set. 
The instruction in this stage guides LLM to focus on the difference in language expression between reference and proper analysis.
This stage helps LLM to perfect the solution and fix the remaining minor mistakes. }
